Understand Data Preprocessing for Effective End-to-End Training of Deep Neural Networks

In this paper, we primarily focus on understanding the data preprocessing pipeline for DNN Training in the public cloud. First, we run experiments to test the performance implications of the two major data preprocessing methods using either raw data or record files. The preliminary results show that data preprocessing is a clear bottleneck, even with the most efficient software and hardware configuration enabled by NVIDIA DALI, a high-optimized data preprocessing library. Second, we identify the potential causes, exercise a variety of optimization methods, and present their pros and cons. We hope this work will shed light on the new co-design of ``data storage, loading pipeline'' and ``training framework'' and flexible resource configurations between them so that the resources can be fully exploited and performance can be maximized.

==> related.tex <==
\section{Related work}
\label{sect:related}

Here, we list and review a set of most relevant work that have been published recently in top-tier conferences.

The articles I have read:\cite{mxnet.record},\cite{hpc.1910.01196},\cite{apple.mldb.10.1145/3299869.3314050},\cite{OneAccess},\cite{1711.03705},\cite{uber.petastorm},\cite{alluxio.Li:EECS-2018-29},\cite{crail.234976},\cite{bigdl.10.1145/3357223.3362707},\cite{file.format},\cite{shuffle.1709.10432}

To be read:\cite{hopsfs.202263},\cite{revisit.1707.02968},\cite{exascale.1909.11150},\cite{parquet.216059}

The articles about data loading pipeline: \cite{hpc.1910.01196},\cite{OneAccess},\cite{streamlining.DNN.ensemble.training.pipelines},\cite{high.performance.data.loading}. \cite{high.performance.data.loading} should be read carefully.


